You Can Have Your Data and Balance It Too: Towards Balanced and Efficient Multilingual Models

Multilingual models have been widely used for cross-lingual transfer to low-resource languages. However, the performance on these languages is hindered by their underrepresentation in the pretraining data. To alleviate this problem, we propose a novel multilingual training technique based on teacher-student knowledge distillation. In this setting, we utilize monolingual teacher models optimized for their language. We use those teachers along with balanced (sub-sampled) data to distill the teachers' knowledge into a single multilingual student. Our method outperforms standard training methods in low-resource languages and retrains performance on high-resource languages while using the same amount of data. If applied widely, our approach can increase the representation of low-resource languages in NLP systems.

==> sections/XX_data_selection.tex <==

We collect a pretraining dataset to train all of ours models on. We aim to represent high and low resource languages, while maintaining a varying set of linguistic features. 

First, we choose two sets of languages. One with shared vocabulary (latin) and another one with distinct vocabulary, as listed in Table~\ref{tab:lang}. These two sets represent a wide variety of languages with diverse typological and morphological features inside of each set. Through our experiments we chose to compare shared and non-shared vocabulary as it has been suggested to be an important factor for multilingual performance \dan{Cite something, and cite ourselves :)}.

Second, We define high resource languages as languages with 50 or 100 million characters, while low resource would have 30,20, or 10 million characters. Figure ~\ref{fig:lang_choice_wiki} shows a comparison of our high-low resource ontology to the existing state in Wikipedia\footnote{Wikipedia dump was obtained and cleaned using wikiextractor~\citep{Wikiextractor2015}.}.

We choose to sample texts from Wikipedia as it consists of roughly similar encyclopedic domain across languages, and is widely used for training PLMs~\citep{devlin-etal-2019-bert}.  
\dan{Not sure where to write about the student balancing, this doesn't seem the right place.}
\begin{figure}[t!]
    \centering
    
    \includegraphics[width=0.45\textwidth]{figures/lang_chart_vs_wiki.png}
    \caption{
    A comparison of high-low resource relation between our choices to Wikipedia, as of May 2022.   \label{fig:lang_choice_wiki}}
\end{figure}

\input{tables/languages}


==> sections/XX_exp_post_hoc_induction.tex <==
We investigate possibility of inducing knowledge for previously unseen languages: Lithuanian (in Latin script group) and Hebrew (in diverse script group).



==> sections/XX_metrics.tex <==
\gabis{I feel like we don't have space for this section in a short paper, I think we have to cram the metrics in the results section}
To evaluate our new approach we focus on two measures. We define a new metric aimed to approximate balanced multilingual language modeling - that is, how skewed a given model is towards high or low resource languages w.r.t to monolingual baselines. Additionally, we evaluate the common measure of cross-lingual transfer using zero-shot evaluation. 
\paragraph{Balanced Multilingual Modeling.}
Since the under-performance of multilingual language models refers to language-specific performances (i.e - being better or worse than the monolingual counterpart) we aim to evaluate our models using a measure that is comprised of per-language evaluations. We measure the performance difference between a given multilingual model and monolingual models associated with the languages in its pre-training set. In other words, for each language $l$ we take an available monolingual model as our gold-standard 
% \footnote{The only language specific criteria for such a model is its performance on the given language. The model itself can utilize whatever data necessary to increase such performance.}
, denoted $\hat{M_l}$, whose performance we want to ideally approximate (or surpass) 
% \footnote{Multilingual pre-trained models are known to suffer from a transfer-interference trade-off\citep{conneau2019unsupervised}, which causes per-language performance to drop as they cover more languages.}
with the multilingual model. Formally, the performance of a multilingual model $M_L$ trained on a language set $L$ and evaluated on $l$, is denoted as: $S_{{M_L}}(l)$. The balanced multilingual performance of $M_L$ on $L$ is defined as $\mathcal{B}$:
\begin{equation}
\label{eq:balanced-modeling}
    \mathcal{B}(M_L,L) \coloneqq \frac{1}{|L|}\sum\limits_{l \in L} (S_{{M_L}}(l)-S_{\hat{M_l}}(l))
\end{equation}

\paragraph{Cross-lingual transfer.}

To measure the cross-lingual transfer of a model $M$ from a language $l_1$ to a language $l_2$ we use the zero-shot transfer score $\mathcal{Z}$ suggested by \citet{hu2020xtreme}  which is defined as:

\begin{equation}
\label{eq:cross-l-score}
    \mathcal{Z}_{M}(l_1,l_2) := S_{M_{\{l_1\}}}(l_2) 
\end{equation}

To measure the cross-lingual performance of a model $M$, across a language set $L$ we report the average zero-shot transfer score on the entire set:
\begin{equation}
\label{eq:avg-cross-l-score}
    \mathcal{C_Z}(M,L) \coloneqq \frac{1}{|L|^2-|L|}\sum\limits_{\substack{l_1,l_2 \in L \\ l_1 \neq l_2}}  \mathcal{Z}_{M}(l_1,l_2)
\end{equation}

\paragraph{Hypotheses.} We hypothesize that our teacher-student setting is more suitable to achieve balanced multilingual performance than the classical methods of training all at once on all available data. Formally, when comparing a student $S$ train  to optimize the languages set $L$ described above to a regular model $B$ trained using cross-entropy on the entire data $D$ we hypothesize \tomasz{train to optimize languages set - what does it mean? }: 
\begin{equation}
\label{eq:balance-hypo}
    \mathcal{B}(B,L)\leq\mathcal{B}(S,L)
\end{equation}

Moreover, we hypothesize that satisfying balanced multilingual modeling might increase cross-lingual transfer:
\begin{equation}
\label{eq:ds-hypo}
 \mathcal{C}_{\mathcal{Z}}(B,L)\leq\mathcal{C}_{\mathcal{Z}}(S,L)
\end{equation}







==> sections/XX_models.tex <==
\subsection{Teacher model}
For all teacher models we train a Masked language modeling only BERT model, without next sentence prediction (Devlin et al., 2019). All teachers were trained with 6 hidden layers and 4 attention heads, an MLM task head, and an embedding dimension of 512. We train a single uncased wordpiece tokenizer (Wu et al., 2016) on the 10mb splits of our entire 14 languages dataset described in section \ref{sec:data}, and additional two 10mb languages: Lithuainian and Hebrew.  We train the models with a batch size of 8 samples, with sentences truncated to 128 tokens. Each language model was trained up to 10 epochs, with early stopping.

\subsection{Student model}


==> tables/ner_f1_res_table.tex <==
\begin{table*}[!bt]
\centering
\small
\begin{tabular}{ll|cc|cc|cc}
\toprule
        &     & \multicolumn{2}{c|}{MLM} & \multicolumn{2}{c|}{MLM balanced} & \multicolumn{2}{c}{Our} \\
        &     & In-Lang & Zero-Shot &      In-Lang & Zero-Shot & In-Lang & Zero-Shot \\
\midrule
\multirow{3}{*}{Shared} & Low-Res &    11.2 &       9.4 &         11.8 &       9.7 &    12.8 &       9.6 \\
        & High-Res &    13.1 &       8.1 &         13.4 &       8.2 &    15.1 &       8.6 \\
        & All &    12.0 &       8.8 &         12.5 &       9.1 &    13.8 &       9.2 \\
\midrule
\multirow{3}{*}{Diverse} & Low-Res &     8.7 &       2.3 &          9.6 &       2.6 &    11.2 &       1.9 \\
        & High-Res &    15.0 &       3.6 &         11.8 &       3.5 &    20.0 &       5.0 \\
        & All &    11.4 &       2.9 &         10.5 &       3.0 &    14.9 &       3.2 \\
\bottomrule
\end{tabular}
\caption{F1 of NER probing. Standard deviations are computed based on 5 runs with different intializations.}
\label{tab:ner-results}
\end{table*}


==> tables/ner_res_f1_table_per_lang.tex <==
\begin{table*}[!tb]
\centering
\small
\begin{tabular}{ll|cc|cc|cc}
\toprule
        &    & \multicolumn{2}{c|}{MLM} & \multicolumn{2}{c|}{MLM balanced} & \multicolumn{2}{c}{Our} \\
        &    &           In-Lang &         Zero-Shot &           In-Lang &         Zero-Shot &           In-Lang &         Zero-Shot \\
\midrule
\multirow{7}{*}{Shared} & de &  14.6 $_{\pm0.8}$ &  10.6 $_{\pm0.6}$ &  14.5 $_{\pm0.9}$ &   9.9 $_{\pm0.8}$ &  15.4 $_{\pm1.3}$ &  10.0 $_{\pm0.9}$ \\
        & en &  10.0 $_{\pm0.2}$ &   7.1 $_{\pm0.4}$ &  11.1 $_{\pm0.7}$ &   7.3 $_{\pm0.7}$ &  12.5 $_{\pm0.7}$ &   7.7 $_{\pm0.8}$ \\
        & es &  14.6 $_{\pm0.7}$ &   6.7 $_{\pm0.6}$ &  14.5 $_{\pm1.3}$ &   7.6 $_{\pm1.0}$ &  17.6 $_{\pm0.8}$ &   8.1 $_{\pm0.7}$ \\
        & eu &  11.6 $_{\pm1.6}$ &  12.5 $_{\pm0.7}$ &   7.1 $_{\pm2.8}$ &  11.8 $_{\pm1.2}$ &  10.1 $_{\pm2.3}$ &  10.1 $_{\pm1.2}$ \\
        & hu &  14.8 $_{\pm1.0}$ &  10.7 $_{\pm1.0}$ &  14.9 $_{\pm1.1}$ &  11.7 $_{\pm0.5}$ &  18.4 $_{\pm0.8}$ &  12.6 $_{\pm1.2}$ \\
        & tr &  12.5 $_{\pm0.8}$ &  10.4 $_{\pm0.8}$ &  17.5 $_{\pm1.1}$ &  10.7 $_{\pm0.5}$ &  14.7 $_{\pm0.8}$ &   9.8 $_{\pm1.0}$ \\
        & vi &   6.0 $_{\pm0.2}$ &   3.8 $_{\pm0.1}$ &   7.7 $_{\pm0.4}$ &   4.6 $_{\pm0.4}$ &   8.1 $_{\pm0.5}$ &   5.9 $_{\pm0.7}$ \\
\cline{1-8}
\multirow{7}{*}{Diverse} & de &  16.0 $_{\pm0.4}$ &   3.2 $_{\pm0.7}$ &  13.0 $_{\pm1.0}$ &   3.4 $_{\pm0.4}$ &  18.8 $_{\pm0.8}$ &   4.7 $_{\pm0.6}$ \\
        & ru &  13.8 $_{\pm0.5}$ &   3.4 $_{\pm0.6}$ &  10.5 $_{\pm0.8}$ &   2.7 $_{\pm0.5}$ &  19.3 $_{\pm0.8}$ &   4.1 $_{\pm0.6}$ \\
        & ko &  15.2 $_{\pm1.0}$ &   4.2 $_{\pm0.3}$ &  11.9 $_{\pm0.9}$ &   4.4 $_{\pm0.4}$ &  21.8 $_{\pm0.9}$ &   6.2 $_{\pm1.5}$ \\
        & el &  12.2 $_{\pm1.0}$ &   4.1 $_{\pm0.5}$ &  11.0 $_{\pm1.3}$ &   5.0 $_{\pm1.2}$ &  17.6 $_{\pm1.0}$ &   3.6 $_{\pm0.4}$ \\
        & hi &   1.7 $_{\pm0.7}$ &   2.2 $_{\pm0.7}$ &   2.0 $_{\pm0.8}$ &   2.1 $_{\pm0.6}$ &   1.1 $_{\pm0.6}$ &   1.8 $_{\pm0.5}$ \\
        & te &   4.6 $_{\pm0.4}$ &   2.8 $_{\pm0.5}$ &   5.0 $_{\pm0.7}$ &   3.0 $_{\pm0.2}$ &   4.1 $_{\pm1.4}$ &   2.0 $_{\pm0.4}$ \\
        & ur &  16.1 $_{\pm0.4}$ &   0.3 $_{\pm0.1}$ &  20.3 $_{\pm0.6}$ &   0.3 $_{\pm0.1}$ &  21.9 $_{\pm1.0}$ &   0.2 $_{\pm0.1}$ \\
\bottomrule
\end{tabular}
\caption{F1 of NER probing for each language. Standard deviations are computed based on 5 runs with different intializations.}
\label{tab:ner-results-all-langs}
\end{table*}


==> tables/pos_significance.tex <==
\begin{table*}
\tiny
\centering
\begin{tabular}{ll|lll|lll|lll|lll}
\toprule
        &          & \multicolumn{6}{c}{MLM} & \multicolumn{6}{c}{MLM balanced} \\
        &          & \multicolumn{3}{c}{In-Lang} & \multicolumn{3}{c}{Zero-Shot} & \multicolumn{3}{c}{In-Lang} & \multicolumn{3}{c}{Zero-Shot} \\
        &          & Our better & Our worse & NS & Our better & Our worse & NS &   Our better & Our worse & NS & Our better & Our worse & NS \\
\midrule
\multirow{2}{*}{Shared} & Low-Res &          1 &         0 &  3 &          3 &         1 &  0 &            0 &         0 &  4 &          2 &         2 &  0 \\
        & High-Res &          2 &         1 &  0 &          0 &         2 &  1 &            3 &         0 &  0 &          2 &         0 &  1 \\
\cline{1-14}
\multirow{2}{*}{Diverse} & Low-Res &          2 &         0 &  2 &          2 &         1 &  1 &            2 &         0 &  2 &          2 &         2 &  0 \\
        & High-Res &          1 &         2 &  0 &          2 &         1 &  0 &            3 &         0 &  0 &          3 &         0 &  0 \\
\bottomrule
% \caption{POS tagging. Number of language with significant improvement or deteriotion over baselines.}
\label{tab:pos-significance}
\end{tabular}
\end{table*}


